Semantic Bound and Multi Types, Revisited

Intersection types are a standard tool in operational and semantical studies of the lambda calculus. De Carvalho showed how multi types, a quantitative variant of intersection types providing a handy presentation of the relational denotational model, allows one to extract precise bounds on the number of $\beta$-steps and the size of normal forms. In the last few years, de Carvalho's work has been extended and adapted to a number of lambda calculi, evaluation strategies, and abstract machines. These works, however, only adapt the first part of his work, that extracts bounds from multi type derivations, while never consider the second part, which deals with extracting bounds from the multi types themselves. The reason is that this second part is more technical, and requires to reason up to type substitutions. It is however also the most interesting, because it shows that the bounding power is inherent to the relational model (which is induced by the types, without the derivations), independently of its presentation as a type system. Here we dissect and clarify the second part of de Carvalho's work, establishing a link with principal multi types, and isolating a key property independent of type substitutions.

==> 09-Complements.tex <==
% !TEX root = main.tex
\section{Complements}
\label{sect:complements}


==> 99-05-Bounds_From_types.tex <==
% !TEX root = main.tex
\section{Proofs of \Cref{sect:bounds-types} (Bounds From Types)}
\label{sect:app-bounds-types}


==> 99-07-Bounds_From_Composable_Types.tex <==
% !TEX root = main.tex
\section{Proofs of \Cref{sect:bounds-comp-types} (Bounds From Composable Types)}
\label{sect:app-bounds-comp-types}


%\begin{lemma}[Normalization and composable types]
%\label{lappendix:norm-and-comppairs-nonempty}
%\NoteState{l:norm-and-comppairs-nonempty}
%Let $\tm$ and $\tmtwo$ be closed terms. Then $\tm\tmtwo$ $\tolo$-normalizes if and only if $\xcompairs\tm\tmtwo \neq \emptyset$. 
%\end{lemma}
%
%\input{\proofspath/leftmost/normalization_composable_bounds}

%\begin{theorem}[Normal form bounds from composable types]
%	\label{thmappendix:nf-bounds-3}
%	\NoteState{thm:nf-bounds-3}
%Let $\tm$ and $\tmtwo$ be closed terms such that there is a normalizing evaluation $\deriv:\tm\tmtwo \tolo^*\nf$.
%\begin{enumerate}
%\item \emph{Lax bounds for all pairs}: $\sksize{\nf} \leq \size\ltype$ for every composable pair $(\tarrow\mtype\ltype, \mtype)\in \xcompairs\tm\tmtwo$. 
%\item \emph{Exact bounds from special pairs}: moreover, $\sksize{\nf} =\size\ltype$ for a composable pair $(\tarrow\mtype\ltype, \mtype)\in \xcompairs\tm\tmtwo$, induced by the pulling back along $\deriv$ of a dry derivation for $\nf$.
%\end{enumerate}
%\end{theorem}
%
%\input{\proofspath/leftmost/nf_composable_bounds}

%\begin{theorem}[Lax bounds from composable types]
%	\label{thmappendix:lax-bounds-3}
%	\NoteState{thm:lax-bounds-3}
%Let $\nf$ and $\nftwo$ be closed normal terms such that $\deriv:\nf\nftwo \tolo^* \nfthree$ with $\nfthree$ normal. Then:
%\begin{enumerate}
%\item \emph{Lax bounds and types}: $2\size{\deriv} + \sksize{\nfthree} \leq \size\ltype+\size\mtype+1$ for every composable pair $(\ltype, \mtype)\in \xcompairs\nf\nftwo$.
%\item \emph{Lax bounds and types, up to substitutions}: $2\size{\deriv} + \sksize{\nfthree} \leq \size\ltype+\size\mtype+1$ for every composable pair up to substitution $(\ltype, \mtype)\in \xsubcompairs\nf\nftwo$.
%\end{enumerate}
%\end{theorem}
%
%\input{\proofspath/leftmost/lax_composable_bounds}

%\begin{theorem}[Exact bounds of kind 3]
%	\label{thmappendix:new-exact-bounds-3}
%	\NoteState{thm:new-exact-bounds-3}
%	Let $\nf$ and $\nftwo$ be normal. 
%	If $\deriv:\nf\nftwo \tolo^* \nfthree$ and $\nfthree$ is normal.
%	\begin{enumerate}
%	\item \emph{Exact bounds}: there 
%	exist $\ltype\in \sem{\nf}$ and $\mtype \in \sem{\nftwo}$ such that $2\size{\deriv} + \sksize\nfthree = 
%	\size\ltype+\size\mtype+1$, and $\ltype$ and $\mtype$ are obtained by drying the composable pair induced by a unitary shrinking derivation for $\nfthree$. 
%	\item \emph{From types composable up to substitution}: moreover, $(\ltype,\mtype)$ are composable up to substitution, that is, $(\ltype,\mtype)\in\xsubcompairs\nf\nftwo$.
%	\end{enumerate}
%\end{theorem}
%
%\input{\proofspath/leftmost/composable_bounds}


==> 99-09-Complements.tex <==
% !TEX root = main.tex
\section{Proofs of \Cref{sect:complements} (Complements)}
\label{sect:app-complements}



==> figure-principal-type-system.tex <==
% !TEX root = main.tex
%\begin{figure}[!t]
 % \centering
 \begin{center}
  \begin{tabular}{c@{\hspace{.5cm}} c@{\hspace{.5cm}} c}
      \AxiomC{}
      \RightLabel{\footnotesize$\ruleAx$}
      \UnaryInfC{$\var \hastype \mset\natype \vdash \var \hastype \patype$}
      \DisplayProof
      &

      \AxiomC{$\ntypctx \vdash \tm \hastype \ptype$}      
      \RightLabel{\footnotesize$\ruleLam$}
      \UnaryInfC{$\ntypctx \sm \var \vdash \la\var\tm\hastype \parrowtype {\ntypctx(\var)} \ptype$}
      \DisplayProof
&

      \AxiomC{$\ntypctx \vdash \tm \hastype \ptype$}
      \RightLabel{\footnotesize$\ruleMany$}
      \UnaryInfC{$\Box_{\nname}\ntypctx \vdash \tm \hastype \Box_{\pname}\ptype$}
      \DisplayProof
            \\\\
                \multicolumn{3}{c}{
	      \AxiomC{$\ntypctx \vdash \tm \hastype  \patype $}
      \AxiomC{$\ntypctxtwo \vdash \tmtwo \hastype \pbtype$}
      \AxiomC{$\patypetwo$ fresh}
      \RightLabel{\footnotesize$\ruleAp$}
      \TrinaryInfC{$(\ntypctx \uplus \ntypctxtwo)\isub\patype{(\parrowtype{\mult\nbtype}{\patypetwo})} \vdash \tm\tmtwo \hastype \patypetwo$}
      \DisplayProof
      }
%     \\\\
%                \multicolumn{3}{c}{
%	      \AxiomC{$\ntypctx \vdash \tm \hastype  \parrowtype\nmtype\ptype $}
%      \AxiomC{$\ntypctxtwo \vdash \tmtwo \hastype \pbtype$}
%      \AxiomC{$\dgreen\sigma \defeq \MGU\nmtype\pbtype$}
%      \RightLabel{\footnotesize$\ruleAp$}
%      \TrinaryInfC{$(\ntypctx \uplus \ntypctxtwo)\dgreen\sigma \vdash \tm\tmtwo \hastype \ptype\dgreen\sigma$}
%      \DisplayProof
%      }
%      \\\\
%      \multicolumn{3}{c}{
%	  \AxiomC{$\ntypctx \vdash \tm \hastype  \ptype $}
%      \AxiomC{$\ntypctxtwo \vdash \tmtwo \hastype \pbtype$}
%      \AxiomC{$\dgreen\sigma \defeq \MGU{\ntypctx(\var)}\pbtype$}
%      \RightLabel{\footnotesize$\ruleES$}
%      \TrinaryInfC{$((\ntypctx \sm\var) \uplus \ntypctxtwo)\dgreen\sigma \vdash \tm\esub\var\tmtwo \hastype \ptype\dgreen\sigma$}
%      \DisplayProof
%      }
    \end{tabular}
%   \medskip
%   \scalebox{0.85}{
%     \begin{prooftree}[label separation=0.3em]%[separation=1.3em]
%     \end{prooftree}
%   }
%  \caption{Silly multi types system.}
%  \label{fig:silly-types}
%\end{figure}
\end{center}


==> figure-shrinking_types.tex <==
% !TEX root = main.tex
\begin{figure*}
\centering
		$\begin{array}{rrcl @{\hspace{.5cm}} rrcl}
		\text{Right  multi type } & \rmtype &\grameq &	\mset{\rltype_1, \dots, \rltype_n} \ \ n \geq 1
		\\
		\text{Right  linear type } & \rltype &\grameq & \ground \mid  \larrow{\lmtype}{\rltype}
		\\
		\text{Left  multi type } & \lmtype &\grameq &	\mset{\lltype_1, \dots, \lltype_n} \ \ n \geq 0
		\\
		\text{Left  linear type } & \lltype &\grameq & \ground \mid  \larrow{\rmtype}{\lltype}
		\\[5pt]
		\text{Unitary right multi type } & \urmtype &\grameq &	\mset{\urltype} 
		\\
		\text{Unitary right linear type } & \urltype &\grameq & \ground \mid  \larrow{\ulmtype}{\urltype}
		\\
		\text{Unitary left multi type } & \ulmtype &\grameq &	\mset{\ulltype_1, \dots, \ulltype_n} \ \ n \geq 0
		\\
		\text{Unitary left linear type } & \ulltype &\grameq & \ground \mid  \larrow{\urmtype}{\ulltype}
		\end{array}$
	\caption{Kinds of right and left (shrinking) types.}
	\label{fig:shrinking}
\end{figure*}

==> proofs/exact_composable_bounds.tex <==
% !TEX root = ../main.tex
\begin{proof}
We show a construction that from any shrinking derivation $\tderiv$ for $\nfthree$ gives types $(\ltype,\mtype)\in\subcompairs(\nf,\nftwo)$ and such that $\size{(\ltype,\mtype)}+1 \geq 
2\size{\deriv} + \sksize{\nfthree}$. The \emph{inf} of the set in the statement is then obtained by taking a  \emph{unitary} shrinking derivation, for which the inequality becomes an equality.

By shrinking completeness (\Cref{thm:shrinking-characterization}), there exists a derivation $\concl{\tderiv}{}{\nf\nftwo}{\ltypetwo}$ such that $\ltypetwo$ is right. By shrinking correctness (\Cref{thm:shrinking-characterization}), $2\size{\deriv} + \sksize{\nfthree} \leq \insize\tderiv$. The 
last rule of $\tderiv$ is an $\ruleAp$ rule, that is, $\tderiv$ has the following shape:
\[
\begin{prooftree}
		\hypo{\tderiv_{\nf}\derives\vdash \nf \hastype \larrow{\mtypetwo}{\ltypetwo}}
		\hypo{\tderiv_{\nftwo} \derives \vdash \nftwo \hastype\mtypetwo}
		\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\nf\nftwo}{}{\ltypetwo}}
\end{prooftree}
\]
for some $\mtypetwo$. Note that $\insize\tderiv = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1$. By dry 
representation up to substitution (\refthm{dry_representation}) applied to $\tderiv_\nf$, there exist a substitution $\sigma_\nf$ and a dry derivation 
$\concl{\tderivtwo_\nf}{}{\nf}{\ltype}$ representing $\tderiv_\nf$, that is, such that $\ltype\sigma_\nf = \larrow{\mtypetwo}{\ltypetwo}$ and 
$\insize{\tderiv_\nf} = \sizetyp{\ltype}$.  Similarly, we obtain a dry derivation $\concl{\tderivtwo_{\nftwo}}{}{\nftwo}{\mtype}$ and a substitution $\sigma_{\nftwo}$ representing $\tderiv_{\nftwo}$, that is, such that  $\mtype\sigma_{\nftwo} = \mtypetwo$ and $\insize{\tderiv_{\nftwo}} = \sizetyp{\mtype}$. 

Note that 
$(\ltype,\mtype)\in\subcompairs(\nf,\nftwo)$ because $\ltype\sigma_\nf = \larrow{\mtypetwo}{\ltypetwo}$ and $\ltypetwo$ is right by hypothesis (because $\tderiv$ is shrinking). 

By stability of dry derivations under renaming (\reflemma{dry-stabile-by-renaming}), we can assume that the supports of $\tderivtwo_\nf$ and $\tderivtwo_{\nftwo}$ are disjoint, so that the domains of $\sigma_\nf$ and $\sigma_{\nftwo}$ are disjoint, allowing us to define $\sigma$ as $\sigma_\nf \cup 
\sigma_{\nftwo}$. 

Additionally (since dry representations are skeletal equivalent, skeletal equivalence preserves the inner size of derivations, and the size of types coincides with the inner size of derivations for dry derivations), 
 $\insize\tderiv = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1 = \sizetyp{\ltype} + 
\sizetyp{\mtype} + 1$, that is, $2\size{\deriv} + \sksize{\nfthree} \leq \insize\tderiv = 
\sizetyp{\ltype} + \sizetyp{\mtype} + 1$.	Now, by starting with a unitary shrinking 
derivation $\tderiv$ for $\nf\nftwo$, by correctness (\Cref{thm:shrinking-characterization}) we obtain 
$2\size{\deriv} + \sksize{\nfthree} = \insize\tderiv$, that is, $2\size{\deriv} + \sksize{\nfthree} 
=\sizetyp{\ltype} + \sizetyp{\mtype} + 1$.\qedhere
\end{proof}

%We conclude with the proof of a corollary of the size representation property  (\Cref{prop:size-representation}.\ref{p:size-representation-fireball}), and not of the previous theorem.
%
%\begin{corollary}[Minimal types catch the size of normal forms]
%	\label{corappendix:minimal-type-normal}
%	\NoteState{cor:minimal-type-normal}
%	Let $\nf$ be a \full fireball. There exists a unitary shrinking derivation $\concl{\tderiv}{\typctx}{\nf}{\mtype}$ such 
%	that $\sizefu{\nf} = \sizetyp{\mtype} + \sizectx{\typctx}$.
%\end{corollary}
%
%\begin{proof}
%	By \refpropp{typability-normal}{fireball}, there exists a unitary shrinking derivation $\derive{\tderivtwo}{\nf}$. 
%	By \Cref{l:size-strong-fireballs}, $\sizefu{\nf} = \insize\tderivtwo$. 
%	By size representation (\Cref{prop:size-representation}.\ref{p:size-representation-fireball}), there 
%	exists $\concl{\tderiv}{\typctx}{\nf}{\mtype}$ such that $\tderiv \tderiveq \tderivtwo$ and $\insize\tderivtwo = \sizetyp{\mtype} + \sizectx{\typctx}$ (thus $\sizefu{\nf} = \sizetyp{\mtype} + \sizectx{\typctx}$).
%	According to $\tderiveq$-invariants (\Cref{l:skel-equiv-properties}), $\tderiv$ is unitary shrinking.
%\end{proof}


==> proofs/head/exact_composable_bounds.tex <==
% !TEX root = ../../main.tex
\begin{proof}
We show a construction that from any derivation $\tderiv$ for $\hnf$ gives types $(\ltype,\mtype)\in\xsubcompairs\nf\nftwo$ and such that $\size{(\ltype,\mtype)}+1 \geq 
2\size{\deriv} + \hdsize{\hnf}$. The \emph{inf} of the set in the statement is then obtained by taking a  \emph{fit} derivation, for which the inequality becomes an equality.

By shrinking completeness (\Cref{thm:shrinking-characterization}), there exists a derivation $\concl{\tderiv}{}{\nf\nftwo}{\ltypetwo}$ such that $\ltypetwo$ is right and $2\size{\deriv} + \hdsize{\hnf} \leq \insize\tderiv$. The 
last rule of $\tderiv$ is an $\ruleAp$ rule, that is, $\tderiv$ has the following shape:
\[
\begin{prooftree}
		\hypo{\tderiv_{\nf}\derives\vdash \tm \hastype \larrow{\mtypetwo}{\ltypetwo}}
		\hypo{\tderiv_{\nftwo} \derives \vdash \tmtwo \hastype\mtypetwo}
		\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\nf\nftwo}{}{\ltypetwo}}
\end{prooftree}
\]
for some $\mtypetwo$. Note that $\insize\tderiv = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1$. By dry 
representation up to substitution (\refthm{dry_representation}) applied to $\tderiv_\nf$, there exist a substitution $\sigma_\nf$ and a dry derivation 
$\concl{\tderivtwo_\nf}{}{\nf}{\ltype}$ representing $\tderiv_\nf$, that is, such that $\ltype\sigma_\nf = \larrow{\mtypetwo}{\ltypetwo}$ and 
$\insize{\tderiv_\nf} = \sizetyp{\ltype}$.  Similarly, we obtain a dry derivation $\concl{\tderivtwo_{\nftwo}}{}{\nftwo}{\mtype}$ and a substitution $\sigma_{\nftwo}$ representing $\tderiv_{\nftwo}$, that is, such that  $\mtype\sigma_{\nftwo} = \mtypetwo$ and $\insize{\tderiv_{\nftwo}} = \sizetyp{\mtype}$. 

By stability of dry derivations under renaming (\reflemma{dry-stabile-by-renaming}), we can assume that the supports of $\tderivtwo_\nf$ and $\tderivtwo_{\nftwo}$ are disjoint, so that the domains of $\sigma_\nf$ and $\sigma_{\nftwo}$ are disjoint, allowing us to define $\sigma$ as $\sigma_\nf \cup 
\sigma_{\nftwo}$. 

Additionally (since dry representations are skeletal equivalent, skeletal equivalence preserves the inner size of derivations, and the size of types coincides with the inner size of derivations for dry derivations), 
 $\insize\tderiv = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1 = \sizetyp{\ltype} + 
\sizetyp{\mtype} + 1$, that is, $2\size{\deriv} + \hdsize{\hnf} \leq \insize\tderiv = 
\sizetyp{\ltype} + \sizetyp{\mtype} + 1$.	Now, by starting with a fit
derivation $\tderiv$ for $\nf\nftwo$, by correctness (\Cref{thm:head-characterization}) we obtain 
$2\size{\deriv} + \hdsize{\hnf} = \insize\tderiv$, that is, $2\size{\deriv} + \hdsize{\hnf} 
=\sizetyp{\ltype} + \sizetyp{\mtype} + 1$.
\end{proof}

%We conclude with the proof of a corollary of the size representation property  (\Cref{prop:size-representation}.\ref{p:size-representation-fireball}), and not of the previous theorem.
%
%\begin{corollary}[Minimal types catch the size of normal forms]
%	\label{corappendix:minimal-type-normal}
%	\NoteState{cor:minimal-type-normal}
%	Let $\nf$ be a \full fireball. There exists a unitary shrinking derivation $\concl{\tderiv}{\typctx}{\nf}{\mtype}$ such 
%	that $\sizefu{\nf} = \sizetyp{\mtype} + \sizectx{\typctx}$.
%\end{corollary}
%
%\begin{proof}
%	By \refpropp{typability-normal}{fireball}, there exists a unitary shrinking derivation $\derive{\tderivtwo}{\nf}$. 
%	By \Cref{l:size-strong-fireballs}, $\sizefu{\nf} = \insize\tderivtwo$. 
%	By size representation (\Cref{prop:size-representation}.\ref{p:size-representation-fireball}), there 
%	exists $\concl{\tderiv}{\typctx}{\nf}{\mtype}$ such that $\tderiv \tderiveq \tderivtwo$ and $\insize\tderivtwo = \sizetyp{\mtype} + \sizectx{\typctx}$ (thus $\sizefu{\nf} = \sizetyp{\mtype} + \sizectx{\typctx}$).
%	According to $\tderiveq$-invariants (\Cref{l:skel-equiv-properties}), $\tderiv$ is unitary shrinking.
%\end{proof}


==> proofs/head/weak_composable_bounds.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By completeness in the head case (\refthm{head-characterization}), there is a fit derivation $\derive{\tderiv}{\nf\nftwo}$ with $2\size{\deriv} + \hdsize{\hnf} = \insize{\tderiv}$. 
	The last rule of $\tderiv$ is an $\ruleAp$ rule between two derivations 
	$\tderiv_\nf$ and $\tderiv_{\nftwo}$. Note that $\insize{\tderiv} = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1$. 
		By dry representation (\refthmp{dry_representation}{core}), there are dry derivations $\concl{\tderiv_\nf'}{\,}{\nf}{\ltype}$ and $\concl{\tderiv_{\nftwo}'}{\,}{\nftwo}{\mtype}$ such that $\tderiv_\nf \tderiveq \tderiv_\nf'$ and $\tderiv_{\nftwo} \tderiveq \tderiv_{\nftwo}'$. By the properties of skeletal invariants (\reflemma{skel-equiv-properties}), $\insize{\tderiv_\nf} = \insize{\tderiv_\nf'}$ and $\insize{\tderiv_{\nftwo}} = \insize{\tderiv_{\nftwo}'}$. By the fact that dry derivations have minimal types (\refprop{dry_is_minimal}), $\insize{\tderiv_\nf'}= \size\ltype$ and $\insize{\tderiv_{\nftwo}'}= \size\mtype$. Putting it all together, we obtain $2\size{\deriv} + \hdsize{\hnf} = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1 = \size\ltype+\size\mtype+1$ with $\ltype\in \sem\nf$ and $\mtype\in\sem\nftwo$.	
\end{proof}

==> proofs/monochromatic_dry_representation.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By induction on the definition of \full inert term and \full fireball. Cases: 
	
	\begin{itemize}
		\item \emph{Variable}, \ie $\tm = \var$. Then $\tderiv$ is a $\ruleManyVar$ rule with $n$ premises $\tderiv_i$ for 
$i\in\set{1,\ldots n}$, which are all axioms, that is, $\sizem{\tderiv_i} = 0$. Therefore $\sizem\tderiv = 0$. If 
$\mtypetwo = \mset{\type_1,\ldots, \type_n}$ then the derivation $\concl{\tderivtwo}{\typctxtwo}{\tm}{\mtypetwo}$ for 
the statement is made out of $n$ axioms of types $\type_1,\ldots, \type_n$ over a $\ruleManyVar$ rule and $\typctxtwo$ 
is simply $\mtypetwo$, so that $\sizectx{\typctxtwo} = \sizetyp{\mtypetwo}$. Then $\tderiv \tderiveq \tderivtwo$ and 
$\sizem{\tderivtwo} = 0 = \sizectx{\typctxtwo} - \sizetyp{\mtypetwo}$.
		

		%%%%%%%%%%%%%%%%%
		\item \emph{Inert application}, \ie $\tm = \sitm \sfire$. Then $\tderiv$ ends with rule $\ruleAp$. Let 
$\tderiv_{\sitm}$ and $\tderiv_{\sfire}$ be its two premises. 		
		By \ih, there is a derivation $\concl{\tderivtwo_{\sfire}}{\typctxtwo_{\sfire}}{\sfire}{\mtypethree}$ such that 
$\tderivtwo_{\sfire} \tderiveq \tderiv_{\sfire}$ and $\sizem{\tderiv_{\sfire}} =  
\sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypethree}$.
		Let $\mtypetwo$ be a multi type such that $\card\mtypetwo = \card\mtype$. Note that rule $\ruleAp$ forces the multi 
type assigned by $\tderiv_{\sitm}$ to $\sitm$ to be a singleton. By \ih, there is a derivation 
$\concl{\tderivtwo_{\sitm}}{\typctxtwo_{\sitm}}{\sitm}{\mset{\larrow{\mtypethree}{\mtypetwo}}}$ such that 
$\tderivtwo_{\sitm} \tderiveq \tderiv_{\sitm}$ and $ 
\sizem{\tderiv_{\sitm}} = \sizectx{\typctxtwo_{\sitm}} - \sizetyp{\mset{\larrow{\mtypethree}{\mtypetwo}}} = 
\sizectx{\typctxtwo_{\sitm}} - 
\sizetyp{\mtypethree} - \sizetyp{\mtypetwo} - 1$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctxtwo_{\sitm} \vdash \sitm \hastype \mset{\larrow{\mtypethree}{\mtypetwo}}}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sfire}$}{\typctxtwo_{\sfire} \vdash \sfire \hastype \mtypethree}
		\infer2[\footnotesize$\ruleAp$]{\typctxtwo_{\sitm}\mplus\typctxtwo_{\sfire} \vdash \sitm\sfire \hastype \mtypetwo}
		\end{prooftree}
		\end{equation*}
		Clearly, $\tderiv \tderiveq \tderivtwo$. Let  $\typctxtwo \defeq \typctxtwo_{\sitm}\mplus\typctxtwo_{\sfire}$. Then 
		\[\small\begin{array}{rcl}
			\sizem\tderiv &= &\sizem{\tderiv_{\sitm}}+ \sizem{\tderiv_{\sfire}} 
+ 1 
			\\
			& =_{\ih} & \sizem{\tderiv_{\sitm}} + \sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypethree} +1
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sitm}} - 
\sizetyp{\mtypethree} - \sizetyp{\mtypetwo} - 1 + \sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypethree} +1
			\\
			& = & \sizectx{\typctxtwo_{\sitm}} + \sizectx{\typctxtwo_{\sfire}} - \sizetyp{\mtypetwo}
			\\
			& = &
			\sizectx\typctxtwo - \sizetyp{\mtypetwo}
		\end{array}\]
		
		For point 2, we use point 1 with $\mtypetwo \defeq \mset{\ground_1, \ldots, \ground_{\card\mtype}}$, for which 
$\sizetyp{\mtypetwo} = 0$, so that equation $\sizem{\tderiv} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo}$ also 
holds true. 
				
		%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on inert}, \ie $\tm = \sitm \esub{\var}{\sitmtwo}$.
		Then $\tderiv$ ends with rule $\ruleES$. Let $\tderiv_{\sitm}$ and $\tderiv_{\sitmtwo}$ be its two premises and Let 
$\mtypetwo$ be a multi type such that $\card\mtypetwo = \card\mtype$.
		By \ih, there is a derivation $\concl{\tderivtwo_{\sitm}}{\typctxtwo_{\sitm}, 
\var\hastype\mtypethree}{\sitm}{\mtypetwo}$ such that $\tderivtwo_{\sitm} \tderiveq \tderiv_{\sitm}$ and 
$\sizem{\tderiv_{\sitm}} = \sizectx{\typctxtwo_{\sitm}, \var\hastype\mtypethree } - \sizetyp{\mtypetwo} = 
\sizectx{\typctxtwo_{\sitm}} + \sizetyp{\mtypethree} - \sizetyp{\mtypetwo}$. By 
\reflemma{skel-equiv-properties}, $\mtypethree$ has the same cardinality of the type $\mtypethree'$ given by 
$\tderiv_{\sitm}$ to $\var$, which is also the same type given by $\tderiv_{\sitmtwo}$ to $\sitmtwo$. We can then apply 
the \ih and obtain a derivation $\concl{\tderivtwo_{\sitmtwo}}{\typctxtwo_{\sitmtwo}}{\sitmtwo}{\mtypethree}$ such that 
$\tderivtwo_{\sitmtwo} \tderiveq \tderiv_{\sitmtwo}$ and $\sizem{\tderiv_{\sitmtwo}} = 
\sizectx{\typctxtwo_{\sitmtwo}} - \sizetyp{\mtypethree}$.
		We have the following derivation $\tderivtwo$:
				\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctxtwo_{\sitm}, \var\hastype\mtypethree \vdash \sitm \hastype \mtypetwo}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitmtwo}$}{\typctxtwo_{\sitmtwo} \vdash \sitmtwo \hastype \mtypethree}
		\infer2[\footnotesize$\ruleES$]{\typctxtwo_{\sitm} \mplus \typctxtwo_{\sitmtwo} \vdash \sitm \esub{\var}{\sitmtwo} 
\hastype \mtypetwo}
		\end{prooftree}
		\end{equation*}
Clearly, $\tderiv \tderiveq \tderivtwo$. Let  $\typctxtwo \defeq \typctxtwo_{\sitmtwo}\mplus\typctxtwo_{\sitm}$. Then 
		\[\small\begin{array}{rcl}
			\sizem\tderiv &=&\sizem{\tderiv_{\sitm}}+ \sizem{\tderiv_{\sitmtwo}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sitm}} + \sizetyp{\mtypethree} - \sizetyp{\mtypetwo} + 
\sizem{\tderiv_{\sitmtwo}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sitm}} + \sizetyp{\mtypethree} - \sizetyp{\mtypetwo} + 
\sizectx{\typctxtwo_{\sitmtwo}} - \sizetyp{\mtypethree} 
			\\
			& = & \sizectx{\typctxtwo_{\sitmtwo}} + \sizectx{\typctxtwo_{\sitm}} - \sizetyp{\mtypetwo}
			\\
			& = &
			\sizectx\typctxtwo - \sizetyp{\mtypetwo}
		\end{array}\]		
				For point 2, we use point 1 with $\mtypetwo \defeq \mset{\ground_1, \ldots, \ground_{\card\mtype}}$, for which 
$\sizetyp{\mtypetwo} = 0$, so that equation $\sizem{\tderiv} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo}$ also 
holds true. 


		%%%%%%%%%%%%%%%%%		
		\item \emph{Abstraction}, \ie $\sfire = \la{\var}{\sfiretwo}$. 
		Then $\tderiv$ ends with a rule $\ruleManyVal$ with $n$ premises, each one ending with a $\ruleFun$ rule. Let 
$\tderiv^i$ be the premise of the $\ruleFun$ rule of the $i$-th derivation above the $\ruleManyVal$ rule, for 
$i\in\set{1,\ldots,n} \eqdef I$.
		By \ih, there exists a derivation $\concl{\tderivtwo^i}{\typctxtwo_i, \var \hastype 
\mtypethree_i'}{\sfiretwo}{\mtypethree_i}$ such that $\tderivtwo^i \tderiveq \tderiv^i$ and $\sizem{\tderiv^i} = 
\sizectx{\typctxtwo_i} + \sizetyp{\mtypethree_i} + \sizetyp{\mtypethree_i'}$.
		We have the following derivation:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo^i$}{\typctxtwo_i, \var \hastype \mtypethree_i' \vdash \sfiretwo \hastype \mtypethree_i}
		
		\infer1[\footnotesize$\lambda$]{\typctxtwo_i \vdash \la{\var}\sfiretwo \hastype 
\larrow{\mtypethree'_i}{\mtypethree_i}}
		\delims{\left[}{\right]_{\iI}}
		\infer1[\footnotesize$\ruleManyVal$]{\uplus_{\iI}\typctxtwo_i \vdash \la{\var}\sfiretwo \hastype 
\mset{\larrow{\mtypethree'_i}{\mtypethree_i}}_{\iI}}		\end{prooftree}
		\end{equation*}
		Clearly, $\tderiv \tderiveq \tderivtwo$. Let $\typctxtwo \defeq \uplus_{\iI}\typctxtwo_i$ and $ \mtypetwo \defeq 
\mset{\larrow{\mtypethree'_i}{\mtypethree_i}}_{\iI}$. We have:
		\[\small\begin{array}{rcl}
			\sizem\tderiv &= &n+\sum_{\iI} \sizem{\tderiv^i}
			\\
			& =_{\ih} & n+\sum_{\iI}(\sizectx{\typctxtwo_i} + \sizetyp{\mtypethree_i} + \sizetyp{\mtypethree_i'}) 
			\\
			& = & \sum_{\iI}\sizectx{\typctxtwo_i} + (n+\sum_{\iI}(\sizetyp{\mtypethree_i} + \sizetyp{\mtypethree_i'}))
			\\
			& = & \sizectx\typctxtwo + \sizetyp{\mset{\larrow{\mtypethree'_i}{\mtypethree_i}}_{\iI}}
			\\
			& = & \sizectx\typctxtwo + \sizetyp\mtypetwo
		\end{array}\]
				
		
		%%%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on fireball}, \ie $\tm = \sfire \esub{\var}{\sitm}$.
		Then $\tderiv$ ends with rule $\ruleES$. Let $\tderiv_{\sfire}$ and $\tderiv_{\sitm}$ be its two premises. 
		By \ih, there is a derivation $\concl{\tderivtwo_{\sfire}}{\typctxtwo_{\sfire}, 
\var\hastype\mtypethree}{\sfire}{\mtypetwo}$ such that $\tderivtwo_{\sfire} \tderiveq \tderiv_{\sfire}$ and 
$\sizem{\tderiv_{\sfire}} = \sizectx{\typctxtwo_{\sfire}} + \size{\mtypethree} + \sizetyp{\mtypetwo}$. By 
\reflemma{skel-equiv-properties}, $\mtypethree$ has the same cardinality of the type $\mtypethree'$ given by 
$\tderiv_{\sfire}$ to $\var$, which is also the same type given by $\tderiv_{\sitm}$ to $\sitm$.
		By \ih, there is a derivation $\concl{\tderivtwo_{\sitm}}{\typctxtwo_{\sitm}}{\sitm}{\mtypethree}$ such that 
$\tderivtwo_{\sitm} \tderiveq \tderiv_{\sitm}$ and $\sizem{\tderiv_{\sitm}} = 
\sizectx{\typctxtwo_{\sitm}} - \sizetyp{\mtypethree}$.
		We have the following derivation $\tderivtwo$:
				\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sfire}$}{\typctxtwo_{\sfire}, \var\hastype\mtypethree \vdash \sfire \hastype \mtypetwo}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctxtwo_{\sitm} \vdash \sitm \hastype \mtypethree}
		\infer2[\footnotesize$\ruleES$]{\typctxtwo_{\sfire} \mplus \typctxtwo_{\sitm} \vdash \sfire \esub{\var}{\sitm} 
\hastype \mtypetwo}
		\end{prooftree}
		\end{equation*}
	Clearly, $\tderiv \tderiveq \tderivtwo$. Let  $\typctxtwo \defeq \typctxtwo_{\sitm}\mplus\typctxtwo_{\sfire}$. Then 
		\[\begin{array}{rcl}
			\sizem\tderiv &= & \sizem{\tderiv_{\sfire}}+ \sizem{\tderiv_{\sitm}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sfire}} + \size{\mtypethree} + \sizetyp{\mtypetwo} + \sizem{\tderiv_{\sitm}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sfire}} + \size{\mtypethree} + \sizetyp{\mtypetwo} + 
\sizectx{\typctxtwo_{\sitm}} 
-\sizetyp{\mtypethree}  
			\\
			& = & \sizectx{\typctxtwo_{\sitm}} + \sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypetwo}
			\\
			& = &
			\sizectx\typctxtwo + \sizetyp{\mtypetwo}
		\end{array}\]
\qedhere
	\end{itemize}	
\end{proof}


==> proofs/open/open-type_size_exists.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By induction on the definition of inert term.
	
	\begin{itemize}
				\item \emph{Variable}, \ie $\tm = \var$. Then $\tderiv$ is a $\ruleManyVar$ rule with $n$ premises $\tderiv_i$ for 
$i\in\set{1,\ldots n}$, which are all axioms. If 
$\imtypetwo = \mset{\inltype_1,\ldots, \inltype_n}$ then the derivation $\concl{\tderivtwo}{\typctxtwo}{\tm}{\imtypetwo}$ for 
the statement is made out of $n$ axioms of types $\inltype_1,\ldots, \inltype_n$ over a $\ruleManyVar$ rule and $\typctxtwo$ 
is simply $\imtypetwo$, so that $\sizectx{\typctxtwo} = \sizetyp{\imtypetwo}$. Then $\tderiv \tderiveq \tderivtwo$.
		

		%%%%%%%%%%%%%%%%%
		\item \emph{Inert application}, \ie $\tm = \itm \fire$ (which is inert). Then $\tderiv$ has the following form. 
		\begin{equation*}
		\tderiv \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctx_{\itm} \vdash \itm \hastype \mset{\larrow{\mtypethree}{\imtype}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctx_{\fire} \vdash \fire \hastype \mtypethree}
		\infer2[\footnotesize$\ruleAp$]{\typctx_{\itm}\mplus\typctx_{\fire} \vdash \itm\fire \hastype \imtype}
		\end{prooftree}
		\end{equation*}
		\ben{Since $\tderiv$ is inert, $\typctx_{\itm}$ are $\typctx_{\fire}$ inert, and by the spreading of inertness (\reflemma{spread-inert}), $\mset{\larrow{\mtypethree}{\imtype}}$ is inert. Then $\tderiv_{\itm}$ is inert, and $\mtypethree$ is a ground multi type. Then $\mset{\larrow{\mtypethree}{\imtypetwo}}$ is also inert.}
By \ih, there is a derivation 
$\concl{\tderivtwo_{\itm}}{\typctxtwo_{\itm}}{\itm}{\mset{\larrow{\mtypethree}{\imtypetwo}}}$ such that 
$\tderivtwo_{\itm} \tderiveq \tderiv_{\itm}$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\itm}$}{\typctxtwo_{\itm} \vdash \itm \hastype \mset{\larrow{\mtypethree}{\imtypetwo}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctx_{\fire} \vdash \fire \hastype \mtypethree}
		\infer2[\footnotesize$\ruleAp$]{\typctxtwo_{\itm}\mplus\typctx_{\fire} \vdash \itm\fire \hastype \imtypetwo}
		\end{prooftree}
		\end{equation*}
		Clearly, $\tderiv \tderiveq \tderivtwo$.
		
		%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on inert}, \ie $\tm = \itm \esub{\var}{\itmtwo}$.
		Then $\tderiv$ has the following form. 
		\begin{equation*}
		\tderiv \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctx_{\itm}, \var\hastype\mtypetwo \vdash \itm \hastype \imtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itmtwo}$}{\typctx_{\itmtwo} \vdash \itmtwo \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\typctx_{\itm} \mplus \typctx_{\itmtwo} \vdash \itm \esub{\var}{\itmtwo} 
\hastype \imtype}
		\end{prooftree}
		\end{equation*}
		with $\typctx = \typctx_{\itm} \mplus \typctx_{\itmtwo}$. \ben{Since $\tderiv$ is inert, $\typctx_{\itm}$ and $\typctx_{\itmtwo}$ are inert, and by the spreading of inertness (\reflemma{spread-inert}), $\mtypetwo$ is inert. Then $\tderiv_{\itm}$ is inert.}
		By \ih, there is a derivation $\concl{\tderivtwo_{\itm}}{\typctxtwo_{\itm}, 
\var\hastype\mtypethree}{\itm}{\imtypetwo}$ such that $\tderivtwo_{\itm} \tderiveq \tderiv_{\itm}$. By 
\reflemma{skel-equiv-properties}, $\mtypethree$ has the same cardinality of the type $\mtypetwo$ given by 
$\tderiv_{\itm}$ to $\var$, which is also the same type given by $\tderiv_{\itmtwo}$ to $\itmtwo$. We can then apply 
the \ih and obtain a derivation $\concl{\tderivtwo_{\itmtwo}}{\typctxtwo_{\itmtwo}}{\itmtwo}{\mtypethree}$ such that 
$\tderivtwo_{\itmtwo} \tderiveq \tderiv_{\itmtwo}$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\itm}$}{\typctxtwo_{\itm}, \var\hastype\mtypethree \vdash \itm \hastype \imtypetwo}
		\hypo{}
		\ellipsis{$\tderivtwo_{\itmtwo}$}{\typctxtwo_{\itmtwo} \vdash \itmtwo \hastype \mtypethree}
		\infer2[\footnotesize$\ruleES$]{\typctxtwo_{\itm} \mplus \typctxtwo_{\itmtwo} \vdash \itm \esub{\var}{\itmtwo} 
\hastype \imtypetwo}
		\end{prooftree}
		\end{equation*}
Clearly, $\tderiv \tderiveq \tderivtwo$. \qedhere
	\end{itemize}	
\end{proof}


==> proofs/open/open-type_size_exists2.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By mutual induction on the definition of inert term and fireball.	
	\begin{itemize}
				\item \emph{Variable}, \ie $\tm = \var$ (which is inert). Then both $\tderiv$ and $\tderivtwo$ are given by a $\ruleManyVar$ rule with $n_\tderiv$ and $n_\tderivtwo$ premises, which are all axioms. Since the multiplicative size of axioms is $0$, we have $\sizem{\tderiv} = 0 = \sizem{\tderivtwo}$. 		

		%%%%%%%%%%%%%%%%%
		\item \emph{Inert application}, \ie $\tm = \itm \fire$ (which is inert). Then $\tderiv$ has the following form. 
		\begin{equation*}
		\tderiv \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctx_{\itm} \vdash \itm \hastype \mset{\larrow{\mtypetwo}{\mtype}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctx_{\fire} \vdash \fire \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleAp$]{\typctx_{\itm}\mplus\typctx_{\fire} \vdash \itm\fire \hastype \mtype}
		\end{prooftree}
		\end{equation*}
		\ben{Since $\tderiv$ is inert, $\typctx_{\itm}$ are $\typctx_{\fire}$ inert, and by the spreading of inertness (\reflemma{spread-inert}), $\mset{\larrow{\mtypetwo}{\mtype}}$ is inert. Then $\tderiv_{\itm}$ is inert, and $\mtypetwo$ is a ground multi type. Then $\tderiv_{\fire}$ is tight.}
		Similarly, $\tderivtwo$ ends with a $\ruleAp$ rule, its premise $\tderivtwo_\itm$ is inert and its premise $\tderivtwo_\fire$ is tight. Then we can apply the \ih (point 1) to $\tderiv_\itm$ and $\tderivtwo_\itm$, and the \ih (point 2) to $\tderiv_\fire$ and $\tderivtwo_\fire$, obtaining $\sizem\tderiv = \sizem{\tderiv_{\itm}}+ \sizem{\tderiv_{\fire}} + 1 =_{\ih} \sizem{\tderivtwo_{\itm}}+ \sizem{\tderivtwo_{\fire}} + 1 = \sizem\tderivtwo$.
		
		%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on inert}, \ie $\tm = \itm \esub{\var}{\itmtwo}$ (which is inert).
		Then necessarily
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \itm \hastype \mtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itmtwo}$}{\typctxthree \vdash \itmtwo \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\itm \esub{\var}{\itmtwo}}{\typctxtwo \mplus \typctxthree}{\mtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is inert, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.} Similarly, $\tderivtwo$ ends with a $\ruleES$ rule, and its two premises $\tderivtwo_\itm$ and $\tderivtwo_{\itmtwo}$ are inert. Then $\sizem\tderiv = \sizem{\tderiv_{\itm}}+ \sizem{\tderiv_{\itmtwo}} =_{\ih} \sizem{\tderivtwo_{\itm}}+ \sizem{\tderivtwo_{\itmtwo}} = \sizem\tderivtwo$.

		%%%%%%%%%%%%%%%%%		
		\item \emph{Abstraction}, \ie $\fire = \la{\var}{\firetwo}$. 
		Both $\tderiv$ and $\tderivtwo$ are tight, that is, they type $\fire$ with a ground multi type. Since they also have to end with a rule $\ruleManyVal$ whose  premises end with a $\ruleFun$ rule, which does not assign a ground type, the only possibility is that both $\ruleManyVal$ rules have $0$ premises and they type $\fire$ with $\zero$. Then $\sizem{\tderiv} = 0 = \sizem{\tderivtwo}$.
						
		
		%%%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on fireball}, \ie $\tm = \fire \esub{\var}{\itm}$. Since $\tderiv$ is tight, it 
has the following shape.
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \fire \hastype \gmtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxthree \vdash \itm \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\fire \esub{\var}{\itm}}{\typctxtwo \mplus \typctxthree}{\gmtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is tight, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.}
Similarly, $\tderivtwo$ ends with a $\ruleES$ rule, its premise $\tderivtwo_\itm$ is inert and its premise $\tderivtwo_\fire$ is tight. Then we can apply the \ih (point 1) to $\tderiv_\itm$ and $\tderivtwo_\itm$, and the \ih (point 2) to $\tderiv_\fire$ and $\tderivtwo_\fire$, obtaining $\sizem\tderiv = \sizem{\tderiv_{\fire}} + \sizem{\tderiv_{\itm}}=_{\ih} \sizem{\tderivtwo_{\fire}} + \sizem{\tderivtwo_{\itm}}= \sizem\tderivtwo$.
\qedhere
	\end{itemize}	
\end{proof}


==> proofs/open/open-type_size_forall.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By mutual induction on the definition of inert term and fireball.
	Note that the statement for the former implies the one for the latter, because if $\tderiv$ is tight then $\imtype$ is a ground multi type, for which $\sizetyp{\imtype} = 0$. Hence for inert terms it is enough to 
	prove \refpoint{open-types-bound-normal-derivations-inert}.
	Cases: 
	\begin{itemize}
		\item \emph{Variable}, \ie~$\tm = \var$ (which is inert). So, necessarily, for some set of indices $I$,
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\infer0[\footnotesize$\ruleAx$]{\tyjp{}{\var}{\var \hastype \mset{\inltype_j}}{\inltype_j}}
		\delims{\left[}{\right]_{\jJ}}
		\infer1[\footnotesize$\ruleManyVar$]{\tyjp{}{\var}{\var \hastype \imtype}{\imtype}}
		\end{prooftree}
		\end{equation*}
		where $\imtype = \mset{\inltype_j}_{\jJ}$ and $\typctx = \var \hastype \imtype$.
		Since $\sizem{\tderiv} = 0$ and $\sizetyp{\imtype} = \sizectx{\typctx}$,
		then $\sizem{\tderiv} = 0 = \sizectx{\typctx}- \sizetyp{\imtype}$.
				
		\item \emph{Application}, \ie~$\tm = \itm \fire$ (which is inert). 
		Then necessarily
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxtwo \vdash \itm \hastype \mult{\larrow{\mtypetwo}{\imtype}}}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctxthree \vdash \fire \hastype\mtypetwo}
		\infer2[\footnotesize$\ruleApp$]{\tyjp{}{\itm \fire}{\typctxtwo \mplus \typctxthree}{\imtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is inert, $\typctxtwo$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mult{\larrow{\mtypetwo}{\imtype}}$ is inert. Therefore, $\mtypetwo$ is a ground multi type and $\tderiv_{\fire}$ is tight}.
		By \ih (point 1 for $\tderiv_{\itm}$, point 2 for $\tderiv_{\fire}$), $\sizem{\tderiv_{\itm}} = \sizectx{\typctxtwo} 
- \sizetyp{\mset{\larrow{\mtypetwo}{\imtype}}} = \sizectx{\typctxtwo} - \sizetyp{\imtype} -1$, because ground multi types have size $0$,  and $\sizem{\tderiv_{\fire}} = 
\sizectx{\typctxthree}$. 
		Therefore, 
		\[\begin{array}{rcl}
		\sizem{\tderiv} & = & \sizem{\tderiv_{\itm}} + \sizem{\tderiv_{\fire}} + 1 
		\\
		& =_{\ih} &\sizectx{\typctxtwo} - \sizetyp{\imtype} -1+ \sizem{\tderiv_{\fire}} + 1  
		\\
		& = &\sizectx{\typctxtwo} - \sizetyp{\imtype}+ \sizem{\tderiv_{\fire}}   
		\\
		& =_{\ih} & \sizectx{\typctxtwo} - \sizetyp{\imtype}+ \sizectx{\typctxthree}
		\\
		& = & \sizectx{\typctx} - \sizetyp{\imtype}.
		\end{array}\]
		
		\item \emph{Explicit substitution on inert}, \ie $\tm = \itm \esub{\var}{\itmtwo}$ (which is inert).
		Then necessarily
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \itm \hastype \imtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itmtwo}$}{\typctxthree \vdash \itmtwo \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\itm \esub{\var}{\itmtwo}}{\typctxtwo \mplus \typctxthree}{\imtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is inert, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.} Therefore both $\tderiv_{\itm}$ and 
$\tderiv_{\itmtwo}$ are inert. 
		By \ih (point 1), $\sizem{\tderiv_{\itm}} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} - \sizetyp{\imtype}$ and $ 
\sizem{\tderiv_{\itmtwo}} = \sizectx{\typctxthree} - \sizetyp{\mtypetwo}$. 
		So, 
		\[\begin{array}{rcl}
		\sizem{\tderiv} & = & \sizem{\tderiv_{\itm}} + \sizem{\tderiv_{\itmtwo}}
		\\
		& =_{\ih} & \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} - \sizetyp{\imtype} + \sizem{\tderiv_{\itmtwo}}
		\\
		& =_{\ih} & \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} - \sizetyp{\imtype} + \sizectx{\typctxthree} - 
\sizetyp{\mtypetwo}
		\\
		& = & \sizectx{\typctxtwo} + \sizectx{\typctxthree} - \sizetyp{\imtype}
		\\
		& = & \sizectx{\typctx} - \sizetyp{\imtype}.
		\end{array}\]
		
		\item \emph{Explicit substitution on fireball}, \ie $\tm = \fire \esub{\var}{\itm}$. Since $\tderiv$ is tight, it 
has the following shape.
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\fire}$}{\typctxtwo, \var \hastype \mtypetwo \vdash \fire \hastype \gmtype}
		\hypo{}
		\ellipsis{$\tderiv_{\itm}$}{\typctxthree \vdash \itm \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\tyjp{}{\fire \esub{\var}{\itm}}{\typctxtwo \mplus \typctxthree}{\gmtype}}
		\end{prooftree}
		\end{equation*}
		where $\typctx = \typctxtwo \mplus \typctxthree$. \ben{Since $\tderiv$ is tight, $\typctxthree$ is inert, and by the 
spreading of inertness (\reflemma{spread-inert}) $\mtypetwo$ is inert.}
		By \ih (point 1 for $\tderiv_{\itm}$, point 2 for $\tderiv_{\fire}$), $\sizem{\tderiv_{\fire}} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} $  and $ \sizem{\tderiv_{\itm}} = 
\sizectx{\typctxthree}-\sizetyp{\mtypetwo}$. 
		Therefore, 
		\[\begin{array}{rcl}
		\size{\tderiv} & = & \sizem{\tderiv_{\fire}} + \sizem{\tderiv_{\itm}}
		\\
		& =_{\ih} & \sizectx{\typctxtwo} + \sizetyp{\mtypetwo} + \sizem{\tderiv_{\itm}}
		\\
		& =_{\ih} & 
		\sizectx{\typctxtwo} + \sizetyp{\mtypetwo} + \sizectx{\typctxthree} - \sizetyp{\mtypetwo}
		\\
		& = & \sizectx{\typctxtwo} + \sizectx{\typctxthree} .
		\\
		& = & \sizectx{\typctx}.
		\end{array}\]
		
		\item \emph{Abstraction}, \ie $\tm = \la{\var}{\tmtwo}$. Since 	$\tderiv$ is tight, it types $\fire$ with a ground multi type. Now, $\tderiv$ also has to end with a rule $\ruleManyVal$, whose premises end with a $\ruleFun$ rule. But $\ruleFun$ does not assign a ground type---the only possibility is that rule $\ruleManyVal$ has $0$ premises and that $\tderiv$ types $\fire$ with $\zero$, as follows.
		\begin{equation*}
		\begin{prooftree}
		\infer0[\footnotesize$\ruleManyVal$]{\vdash \la{\var}\fire \hastype \zero}		
		\end{prooftree}
		\end{equation*}
		Then $\typctx$ is empty and $\sizem\tderiv = 0 = \sizectx\typctx$.
		\qedhere
	\end{itemize}
\end{proof}


==> proofs/refined_composable_bounds.tex <==
% !TEX root = ../main.tex
\begin{proof}
\hfill
\begin{enumerate}
\item
\end{enumerate}
\end{proof}



==> proofs/strong/strong-type_size_exists-refined.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By mutual induction on the definition of \full inert term and \full fireball. Cases: 
	
	\begin{itemize}
		\item \emph{Variable}, \ie $\tm = \var$. Then $\tderiv$ has the following shape:
		\begin{equation*}
		\tderiv =
		\begin{prooftree}
		\hypo{\left[\var \hastype \mset{\type_i} \vdash^\infty \var \hastype \type_i\right]_{i\in\set{1,\ldots, n}}}
		\infer1[\footnotesize$\ruleManyVar$]{\var\hastype\mtype \vdash^\infty \var \hastype \mtype}		\end{prooftree}
		\end{equation*}
		with $\mtype = \mset{\type_1,\ldots, \type_n}$ and $\typctx$ being simply $\var\hastype \mtype$. Note that 
$\sizem{\tderiv} = 0$. Take $\mtype' \defeq \mset{\ground_{i_1},\ldots, \ground_{i_n}}$ with $\ground_{i_1},\ldots, 
\ground_{i_n}$ fresh variables with respect to $\groundset$ (thus in particular not appearing in $\type_1,\ldots, 
\type_n$). Then the derivation $\conclin{\tderivtwo}{\typctx'}{\tm}{\mtype'}$ for the statement is:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{\left[\var \hastype \mset{\ground_i} \vdash^\infty \var \hastype \ground_i\right]_{i\in\set{1,\ldots, n}}}
		\infer1[\footnotesize$\ruleManyVar$]{\var\hastype\mtype' \vdash^\infty \var \hastype \mtype'}		\end{prooftree}
		\end{equation*}
		with $\typctx'$ being simply $\var\hastype\mtype'$. The substitution is $\sigma \defeq 
\isub{\ground_{i_1}}{\type_1}\ldots \isub{\ground_{i_n}}{\type_n}$. 
		\begin{itemize}
			\item \emph{Skeleton}: clearly, $\tderiv \tderiveq \tderivtwo$. 
			\item \emph{Representation}: clearly, $\sigma(\mtypetwo) = \mtype$, that implies $\sigma(\tderivtwo) = \tderiv$.
			\item \emph{Reinforced disjoint names}: by construction the ground types in $\gt{\tderivtwo}= 
\set{\ground_{i_1},\ldots, \ground_{i_n}}$ are not in $\groundset$.
			\item \emph{Types size}: $\sizem{\tderivtwo} = 0 = \sizetyp{\mtype'} - \sizetyp{\mtype'} = \sizectx{\typctx'} - 
\sizetyp{\mtype'}$
		\end{itemize}
		
		For point 2, simply note that $\sizem{\tderivtwo} = 0 = \sizetyp{\mtype'} + \sizetyp{\mtype'} = \sizectx{\typctx'} + 
\sizetyp{\mtype'}$.

		%%%%%%%%%%%%%%%%%
				\item \emph{Inert application}, \ie $\tm = \sitm \sfire$. Then $\tderiv$ ends with rule $\ruleAp$:
		\begin{equation*}
		\tderiv =
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\sitm}$}{\typctx_{\sitm} \vdash^\infty \sitm \hastype \mset{\larrow{\mtypetwo}{\mtype}}}
		\hypo{}
		\ellipsis{$\tderiv_{\sfire}$}{\typctx_{\sfire} \vdash^\infty \sfire \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleAp$]{\typctx_{\sitm}\mplus\typctx_{\sfire} \vdash^\infty \sitm\sfire \hastype \mtype}
		\end{prooftree}
		\end{equation*}
		with $\typctx = \typctx_{\sitm}\mplus\typctx_{\sfire}$.
		By \ih (point 2) with respect to $\groundsettwo \defeq \groundset \cup \dom\tau$, there exist a substitution 
$\sigma_{\sfire}$ and derivation $\conclin{\tderivtwo_{\sfire}}{\typctx'_{\sfire}}{\sfire}{\mtypetwo'}$ such that they 
form a size dissection of $\tderiv_{\sfire}$ such that $\gt{\tderivtwo_{\sfire}}\cap \groundsettwo = \emptyset$.
		
		Consider now the type $\mset{\larrow{\mtypetwo'}{\mtype'}}$. Because of the properties given by the \ih above, we 
have that $\sigma_{\sfire}(\tau(\mset{\larrow{\mtypetwo'}{\mtype'}})) = 
\mset{\larrow{\sigma_{\sfire}(\mtypetwo')}{\tau(\mtype')}} = \mset{\larrow{\mtypetwo}{\mtype}}$. Let $\tau'$ be 
$\sigma_{\sfire}\comp\tau |_{\gt{\mset{\larrow{\mtypetwo'}{\mtype'}}}}$, that is the restriction of 
$\sigma_{\sfire}\comp\tau$ to the ground types in $\mset{\larrow{\mtypetwo'}{\mtype'}}$. By \ih (point 1) with respect 
to $\groundsetthree \defeq \groundset \cup (\dom{\sigma_{\sfire}} \setminus \gt{\mtypetwo'})$, there exist a 
substitution $\sigma_{\sitm}$ extending $\tau'$ and a derivation 
$\conclin{\tderivtwo_{\sitm}}{\typctx'_{\sitm}}{\sitm}{\mset{\larrow{\mtypetwo'}{\mtype'}}}$ forming a dissection of 
$\tderiv_{\sitm}$ such that $\sizem{\tderiv_{\sitm}} = \sizectx{\typctx'_{\sitm}} - 
\sizetyp{\mset{\larrow{\mtypetwo'}{\mtype'}}} = \sizectx{\typctx'_{\sitm}} - \sizetyp{\mtypetwo'} - \sizetyp{\mtype'} 
-1$ and $\gt{\tderivtwo_{\sitm}}\cap \groundsetthree = \emptyset$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctx'_{\sitm} \vdash^\infty \sitm \hastype \mset{\larrow{\mtypetwo'}{\mtype'}}}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sfire}$}{\typctx'_{\sfire} \vdash^\infty \sfire \hastype \mtypetwo'}
		\infer2[\footnotesize$\ruleAp$]{\typctx'_{\sitm}\mplus\typctx'_{\sfire} \vdash^\infty \sitm\sfire \hastype \mtype'}
		\end{prooftree}
		\end{equation*}
		Let $\sigma \defeq \sigma_{\sfire} \comp \sigma_{\sitm}$. We have to show that $(\tderivtwo, \sigma)$ is a 
dissection satisfying the statement of point 1.
		\begin{itemize}
			\item \emph{Skeleton}: the two \ih give $\tderiv_{\sfire} \tderiveq \tderivtwo_{\sfire}$ and $\tderiv_{\sitm} 
\tderiveq \tderivtwo_{\sitm}$, that imply $\tderiv \tderiveq \tderivtwo$. 

			\item \emph{Representation}: by choice of $\groundsettwo$ and $\groundsetthree$, $\dom{\sigma_{\sfire}} 
\cap\dom{\sigma_{\sitm}} = \gt{\mtypetwo'}$, on which they agree because $\sigma_{\sitm}$ extends $\tau'$, that is, 
$\sigma = \sigma_{\sfire}$ on $\dom{\sigma_{\sfire}}$ and similarly for $\sigma_{\sitm}$. Then 
$\sigma(\tderivtwo_{\sfire}) = \sigma_{\sfire}(\tderivtwo_{\sfire}) =_{\ih} \tderiv_{\sfire}$ and similarly 
$\sigma(\tderivtwo_{\sfire}) = \tderiv_{\sfire}$, that is, $\sigma(\tderivtwo) = \tderiv$.
			\item \emph{Reinforced disjoint names}: we have that $\gt{\tderivtwo_{\sfire}}\cap \groundsettwo = \emptyset$ and 
$\gt{\tderivtwo_{\sitm}}\cap \groundsetthree = \emptyset$. Since both $\groundsettwo$ and $\groundsetthree$ contain 
$\groundset$, we have that the reinforced disjoint names requirement holds: $\gt{\tderivtwo}\cap \groundset = 
(\gt{\tderivtwo_{\sfire}}\cup \gt{\tderivtwo_{\sitm}} )\cap \groundset = (\gt{\tderivtwo_{\sfire}}\cap \groundset)\cup 
(\gt{\tderivtwo_{\sitm}} \cap \groundset) = \emptyset \cup \emptyset = \emptyset$.
			\item \emph{Types size}: let  $\typctx' \defeq \typctx'_{\sitm}\mplus\typctx'_{\sfire}$. Then 
		\[\small\begin{array}{rcl}
			\sizem\tderiv &= & \sizem{\tderiv_{\sitm}}+ \sizem{\tderiv_{\sfire}} + 1
			\\
			& =_{\ih} & \sizem{\tderiv_{\sitm}} + \sizectx{\typctx'_{\sfire}} + \sizetyp{\mtypetwo'} + 1
			\\
			& =_{\ih} & \sizectx{\typctx'_{\sitm}} - \sizetyp{\mtypetwo'} - \sizetyp{\mtype'} -1 + \sizectx{\typctx'_{\sfire}} 
+ \sizetyp{\mtypetwo'} + 1
			\\			
			& = & \sizectx{\typctx'_{\sitm}} + \sizectx{\typctx'_{\sfire}} -\sizetyp{\mtype'}
			\\
			& = & \sizectx\typctx' -\sizetyp{\mtype'}.
		\end{array}\]
		\end{itemize}
		
		For point 2, if $\mtype = \mset{\type_1, \ldots, \type_{\card\mtype}}$ we use point 1 with $\mtype' \defeq 
\mset{\ground_{i_1}, \ldots, \ground_{i_{\card\mtype}}}$ where $\ground_{i_1}, \ldots, \ground_{i_{\card\mtype}}$ are 
not in $\gt\tderiv$, and $\tau \defeq \isub{\ground_{i_1}}{\type_1}\ldots 
\isub{\ground_{i_{\card\mtype}}}{\type_{\card\mtype}}$---clearly $\tau$ is a substitution such that $\tau(\mtype') = 
\mtype$ and $\dom\tau=\gt{\mtype'}$. Note that $\sizetyp{\mtype'} = 0$, so that equation $\sizem{\tderiv} =  
\sizectx{\typctx'} + \sizetyp{\mtype'}$ also holds true. 
				
		%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on inert}, \ie $\tm = \sitm \esub{\var}{\sitmtwo}$.
		Then $\tderiv$ ends with rule $\ruleES$:
		\begin{equation*}
		\tderiv =
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\sitm}$}{\typctx_{\sitm}, \var\hastype\mtypetwo \vdash^\infty \sitm \hastype \mtype}
		\hypo{}
		\ellipsis{$\tderiv_{\sitmtwo}$}{\typctx_{\sitmtwo} \vdash^\infty \sitmtwo \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\typctx_{\sitm} \mplus \typctx_{\sitmtwo} \vdash^\infty \sitm \esub{\var}{\sitmtwo} 
\hastype \mtype}
		\end{prooftree}
		\end{equation*}
		Let $\mtype'$ and $\tau$ be such that $\tau(\mtype') = \mtype$ and $\dom\tau = \gt{\mtype'}$.
By \ih (point 1), there exist a substitution $\sigma_{\sitm}$ extending $\tau$ and a derivation 
$\conclin{\tderivtwo_{\sitm}}{\typctx'_{\sitm}, \var\hastype\mtypetwo'}{\sitm}{\mtype'}$ forming a dissection of 
$\tderiv_{\sitm}$ such that $\sizem{\tderiv_{\sitm}} = \sizectx{\typctx'_{\sitm}} +\sizetyp{\mtypetwo'} - 
\sizetyp{\mtype'}$ and $\gt{\tderivtwo_{\sitm}}\cap \groundset = \emptyset$.


		Let $\sigma_{\mtypetwo'}$ be the restriction of $\sigma_{\sitm}$ to $\gt{\mtypetwo'}$. By \ih (point 1) with respect 
to $\groundsettwo \defeq \groundset \cup (\dom{\sigma_{\sitm}} \setminus \gt{\mtypetwo'})$, there exist a substitution 
$\sigma_{\sitmtwo}$ extending $\sigma_{\mtypetwo'}$ and a derivation 
$\conclin{\tderivtwo_{\sitmtwo}}{\typctx'_{\sitmtwo}}{\sitmtwo}{\mtypetwo'}$ forming a dissection of 
$\tderiv_{\sitmtwo}$ such that $\sizem{\tderiv_{\sitmtwo}} = \sizectx{\typctx'_{\sitmtwo}} - \sizetyp{\mtypetwo'}$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctx'_{\sitm}, \var\hastype\mtypetwo' \vdash^\infty \sitm \hastype \mtype'}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitmtwo}$}{\typctx'_{\sitmtwo} \vdash^\infty \sitmtwo \hastype \mtypetwo'}
		\infer2[\footnotesize$\ruleES$]{\typctx'_{\sitm} \mplus \typctx'_{\sitmtwo} \vdash^\infty \sitm 
\esub{\var}{\sitmtwo} \hastype \mtype'}
		\end{prooftree}
		\end{equation*}
		\begin{itemize}
			\item \emph{Skeleton}: the two \ih give $\tderiv_{\sitm} \tderiveq \tderivtwo_{\sitm}$ and $\tderiv_{\sitmtwo} 
\tderiveq \tderivtwo_{\sitmtwo}$, that imply $\tderiv \tderiveq \tderivtwo$. 
			\item \emph{Representation}: by choice of $\groundsettwo$, $\dom{\sigma_{\sitm}} \cap\dom{\sigma_{\sitmtwo}} = 
\gt{\mtypetwo'}$, on which they agree because $\sigma_{\sitm}$ extends $\sigma_{\mtypetwo'}$, that is, $\sigma = 
\sigma_{\sitm}$ on $\dom{\sigma_{\sitm}}$ and similarly for $\sigma_{\sitmtwo}$. Then $\sigma(\tderivtwo_{\sitm}) = 
\sigma_{\sitm}(\tderivtwo_{\sitm}) =_{\ih} \tderiv_{\sitm}$ and similarly $\sigma(\tderivtwo_{\sitmtwo}) = 
\tderiv_{\sitmtwo}$, that is, $\sigma(\tderivtwo) = \tderiv$.
			\item \emph{Reinforced disjoint names}: we have that $\gt{\tderivtwo_{\sitm}}\cap \groundset = \emptyset$ and 
$\gt{\tderivtwo_{\sitmtwo}}\cap \groundsettwo = \emptyset$. Since $\groundsettwo$ contains $\groundset$, we have that 
the reinforced disjoint names requirement holds: $\gt{\tderivtwo}\cap \groundset = (\gt{\tderivtwo_{\sitm}}\cup 
\gt{\tderivtwo_{\sitmtwo}} )\cap \groundset = (\gt{\tderivtwo_{\sitm}}\cap \groundset)\cup (\gt{\tderivtwo_{\sitmtwo}} 
\cap \groundset) = \emptyset \cup \emptyset = \emptyset$.
			\item \emph{Types size}: let  $\typctx' \defeq \typctx'_{\sitm}\mplus\typctx'_{\sitmtwo}$. Then 
		\[\small\begin{array}{rcl}
			\sizem\tderiv &= &\sizem{\tderiv_{\sitm}}+ \sizem{\tderiv_{\sitmtwo}} 
			\\
			& =_{\ih} &\sizem{\tderiv_{\sitm}} + \sizectx{\typctx'_{\sitmtwo}} - \sizetyp{\mtypetwo'}
			\\
			& =_{\ih} & \sizectx{\typctx'_{\sitm}} +\sizetyp{\mtypetwo'} - \sizetyp{\mtype'} + \sizectx{\typctx'_{\sitmtwo}} - 
\sizetyp{\mtypetwo'}
			\\
			& = & \sizectx{\typctx'_{\sitmtwo}} + \sizectx{\typctx'_{\sitm}} - \sizetyp{\mtype'}
			\\
			& = & \sizectx{\typctx'}- \sizetyp{\mtype'}
		\end{array}\]		
		\end{itemize}
		
		For point 2, if $\mtype = \mset{\type_1, \ldots, \type_{\card\mtype}}$ we use point 1 with $\mtype' \defeq 
\mset{\ground_{i_1}, \ldots, \ground_{i_{\card\mtype}}}$ where $\ground_{i_1}, \ldots, \ground_{i_{\card\mtype}}$ are 
not in $\gt\tderiv$, and $\tau \defeq \isub{\ground_{i_1}}{\type_1}\ldots 
\isub{\ground_{i_{\card\mtype}}}{\type_{\card\mtype}}$---clearly $\tau$ is a substitution such that $\tau(\mtype') = 
\mtype$ and $\dom\tau=\gt{\mtype'}$. Note that $\sizetyp{\mtype'} = 0$, so that equation $\sizem{\tderiv} =  
\sizectx{\typctx'} + \sizetyp{\mtype'}$ also holds true. 


		%%%%%%%%%%%%%%%%%		
		\item \emph{Abstraction}, \ie $\sfire = \la{\var}{\sfiretwo}$. 
		Then $\tderiv$ has the following shape, for some $n\in\nat$. 
		\begin{equation*}
		\tderiv =
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv^i$}{\typctx_i, \var \hastype \mtypethree_i \vdash^\infty \sfiretwo \hastype \mtypetwo_i}
		
		\infer1[\footnotesize$\lambda$]{\typctx_i \vdash^\infty \la{\var}\sfiretwo \hastype 
\larrow{\mtypethree_i}{\mtypetwo_i}}
		\delims{\left[}{\right]_\iN}
		\infer1[\footnotesize$\ruleManyVal$]{\uplus_\iN\typctx_i \vdash^\infty \la{\var}\sfiretwo \hastype 
\mset{\larrow{\mtypethree_i}{\mtypetwo_i}}_\iN}		
		\end{prooftree}
		\end{equation*}
		with $\typctx \defeq \uplus_\iN\typctx_i$ and $ \mtype \defeq \mset{\larrow{\mtypethree_i}{\mtypetwo_i}}_\iN$. 
		
		By \ih (point 2) with respect to $\groundset_1 \defeq \groundset$, there exists a substitution 
$\sigma_{\tderivtwo^1}$ and a derivation $\conclin{\tderivtwo^1}{\typctx'_1, \var \hastype 
\mtypethree_1'}{\sfiretwo}{\mtypetwo_1'}$ forming a size dissection for $\tderiv^1$ such that $\sizem{\tderivtwo^1} = 
\sizectx{\typctx'_1,\var \hastype \mtypethree_1'} + \sizetyp{\mtypetwo_1'} = \sizectx{\typctx'_1} + 
\sizetyp{\mtypethree_1'} + \sizetyp{\mtypetwo_1'}$. Applying again the \ih (point 2) with respect to $\groundset_2 
\defeq \groundset \cup \dom{\sigma_{\tderivtwo^1}}$ we obtain a similar size dissection for $\tderiv^2$. Iterating with 
respect to $\groundset_i \defeq \groundset \cup \dom{\sigma_{\tderivtwo^1}}\cup\mydots \cup 
\dom{\sigma_{\tderivtwo^{i-1}}}$, we obtain size dissections for all $\tderiv^i$.
		We then have the following derivation:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo^i$}{\typctx'_i, \var \hastype \mtypethree'_i \vdash^\infty \sfiretwo \hastype \mtypetwo'_i}
		
		\infer1[\footnotesize$\lambda$]{\typctx'_i \vdash^\infty \la{\var}\sfiretwo \hastype 
\larrow{\mtypethree'_i}{\mtypetwo'_i}}
		\delims{\left[}{\right]_\iN}
		\infer1[\footnotesize$\ruleManyVal$]{\uplus_\iN\typctx'_i \vdash^\infty \la{\var}\sfiretwo \hastype 
\mset{\larrow{\mtypethree'_i}{\mtypetwo'_i}}_\iN}		
		\end{prooftree}
		\end{equation*}
Let $\typctx' \defeq \uplus_\iN\typctx'_i$ and $ \mtype' \defeq \mset{\larrow{\mtypethree'_i}{\mtypetwo'_i}}_\iN$. 		
\begin{itemize}
			\item \emph{Skeleton}: by \ih $\tderiv^i \tderiveq \tderivtwo^i$. Then, $\tderiv \tderiveq \tderivtwo$. 
			\item \emph{Representation}: by choice of $\groundset_i$, the substitutions $\sigma_{\tderiv^i}$ have pairwise 
disjoint domains. Then $\sigma = \sigma_{\tderiv^i}$ on $\dom{\sigma_{\tderiv^i}}$. Then $\sigma(\tderivtwo^i) = 
\sigma_{\tderivtwo^i}(\tderivtwo^i) =_{\ih} \tderiv^i$, that is, $\sigma(\tderivtwo) = \tderiv$.
			\item \emph{Reinforced disjoint names}: by choice of $\groundset_i$, we have that $\gt{\tderivtwo^i}\cap 
\groundset = \emptyset$ for all $i$. Then, $\gt{\tderivtwo}\cap \groundset = (\cup_\iN\gt{\tderivtwo^i})\cap \groundset 
= \cup_\iN(\gt{\tderivtwo^i}\cap \groundset) = \cup_\iN\emptyset = \emptyset$.
			\item \emph{Types size}: we have:
		\[\small\begin{array}{rcl}
			\sizem\tderiv &= &n+\sum_\iN \sizem{\tderiv^i}
			\\
			& =_{\ih} & n+\sum_\iN(\sizectx{\typctx'_i} + \sizetyp{\mtypethree_i'} + \sizetyp{\mtypetwo'_i}) 
			\\
			& = & \sum_\iN\sizectx{\typctx'_i} + (\sum_\iN(\sizetyp{\mtypethree_i'} + \sizetyp{\mtypetwo'_i} +1))
			\\
			& = & \sizectx\typctx' + \sizetyp{\mset{\larrow{\mtypethree'_i}{\mtypetwo'_i}}_\iN}
			\\
			& = & \sizectx\typctx' + \sizetyp{\mtype'}
		\end{array}\]
		\end{itemize}
						
		
		%%%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on fireball}, \ie $\tm = \sfire \esub{\var}{\sitm}$.
		Then $\tderiv$ ends with rule $\ruleES$:
		\begin{equation*}
		\tderiv = 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderiv_{\sfire}$}{\typctx_{\sfire}, \var\hastype\mtypetwo \vdash^\infty \sfire \hastype \mtype}
		\hypo{}
		\ellipsis{$\tderiv_{\sitm}$}{\typctx_{\sitm} \vdash^\infty \sitm \hastype \mtypetwo}
		\infer2[\footnotesize$\ruleES$]{\typctx_{\sfire} \mplus \typctx_{\sitm} \vdash^\infty \sfire \esub{\var}{\sitm} 
\hastype \mtype}
		\end{prooftree}
		\end{equation*}
		with $\typctx \defeq \typctx_{\sfire}\mplus\typctx_{\sitm}$.
		By \ih (point 2), there is a substitution $\sigma_{\sfire}$ and a derivation 
$\conclin{\tderivtwo_{\sfire}}{\typctx'_{\sfire}, \var\hastype\mtypetwo'}{\sfire}{\mtype'}$ forming a size dissection of 
$\tderiv_{\sfire}$ such that $\gt{\tderivtwo_{\sfire}} \cap \groundset = \emptyset$. 
		Let $\sigma_{\mtypetwo'}$ the restriction of $\sigma_{\sfire}$ to $\gt{\mtypetwo'}$.
		By \ih (point 1) with respect to $\groundsettwo \defeq \groundset \cup (\dom{\sigma_{\sfire}} \setminus 
\gt{\mtypetwo'})$, there is a substitution $\sigma_{\sitm}$ extending $\sigma_{\mtypetwo'}$ and a derivation 
$\conclin{\tderivtwo_{\sitm}}{\typctx'_{\sitm}}{\sitm}{\mtypetwo'}$ forming a dissection of $\tderiv_{\sitm}$ such that 
$\sizem{\tderiv_{\sitm}} = \sizectx{\typctx'_{\sitm}}-\sizetyp{\mtypetwo'}$ and $\gt{\tderivtwo_{\sitm}} \cap 
\groundsettwo = \emptyset$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sfire}$}{\typctx'_{\sfire}, \var\hastype\mtypetwo' \vdash^\infty \sfire \hastype \mtype'}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctx'_{\sitm} \vdash^\infty \sitm \hastype \mtypetwo'}
		\infer2[\footnotesize$\ruleES$]{\typctx'_{\sfire} \mplus \typctx'_{\sitm} \vdash^\infty \sfire \esub{\var}{\sitm} 
\hastype \mtype'}
		\end{prooftree}
		\end{equation*}
		\begin{itemize}
			\item \emph{Skeleton}: the two \ih give $\tderiv_{\sfire} \tderiveq \tderivtwo_{\sfire}$ and $\tderiv_{\sitm} 
\tderiveq \tderivtwo_{\sitm}$, that imply $\tderiv \tderiveq \tderivtwo$. 
			\item \emph{Representation}: by choice of $\groundsettwo$, $\dom{\sigma_{\sfire}} \cap\dom{\sigma_{\sitm}} = 
\gt{\mtypetwo'}$, on which they agree because $\sigma_{\sitm}$ extends $\sigma_{\mtypetwo'}$, that is, $\sigma = 
\sigma_{\sfire}$ on $\dom{\sigma_{\sfire}}$ and similarly for $\sigma_{\sitm}$. Then $\sigma(\tderivtwo_{\sfire}) = 
\sigma_{\sfire}(\tderivtwo_{\sfire}) =_{\ih} \tderiv_{\sfire}$ and similarly $\sigma(\tderivtwo_{\sitm}) = 
\tderiv_{\sitm}$, that is, $\sigma(\tderivtwo) = \tderiv$.

			\item \emph{Reinforced disjoint names}: we have that $\gt{\tderivtwo_{\sfire}}\cap \groundset = \emptyset$ and 
$\gt{\tderivtwo_{\sitm}}\cap \groundsettwo = \emptyset$. Since $\groundsettwo$ contains $\groundset$, we obtain: 
$\gt{\tderivtwo}\cap \groundset = (\gt{\tderivtwo_{\sfire}}\cup \gt{\tderivtwo_{\sitm}} )\cap \groundset = 
(\gt{\tderivtwo_{\sfire}}\cap \groundset)\cup (\gt{\tderivtwo_{\sitm}} \cap \groundset) = \emptyset \cup \emptyset = 
\emptyset$.

			\item \emph{Types size}: let  $\typctx' \defeq \typctx'_{\sfire}\mplus\typctx'_{\sitm}$. Then 
		\[\begin{array}{rcl}
			\sizem\tderiv &= & \sizem{\tderiv_{\sfire}}+ \sizem{\tderiv_{\sitm}} 
			\\
			& =_{\ih} & \sizectx{\typctx'_{\sfire}} + \size{\mtypetwo'} + \sizetyp{\mtype'} + \sizem{\tderiv_{\sitm}} 
			\\
			& =_{\ih} & \sizectx{\typctx'_{\sfire}} + \size{\mtypetwo'} + \sizetyp{\mtype'} + \sizectx{\typctx'_{\sitm}} 
-\sizetyp{\mtypetwo'}  
			\\
			& = & \sizectx{\typctx'_{\sitm}} + \sizectx{\typctx'_{\sfire}} + \sizetyp{\mtype'}
			\\
			& = &
			\sizectx{\typctx'} + \sizetyp{\mtype'}
		\end{array}\]
		\end{itemize}
		
\qedhere
	\end{itemize}	
\end{proof}


==> proofs/strong/strong-type_size_exists.tex <==
% !TEX root = ../../main.tex
\begin{proof}
	By induction on the definition of \full inert term and \full fireball. Cases: 
	
	\begin{itemize}
		\item \emph{Variable}, \ie $\tm = \var$. Then $\tderiv$ is a $\ruleManyVar$ rule with $n$ premises $\tderiv_i$ for 
$i\in\set{1,\ldots n}$, which are all axioms, that is, $\sizem{\tderiv_i} = 0$. Therefore $\sizem\tderiv = 0$. If 
$\mtypetwo = \mset{\type_1,\ldots, \type_n}$ then the derivation $\concl{\tderivtwo}{\typctxtwo}{\tm}{\mtypetwo}$ for 
the statement is made out of $n$ axioms of types $\type_1,\ldots, \type_n$ over a $\ruleManyVar$ rule and $\typctxtwo$ 
is simply $\mtypetwo$, so that $\sizectx{\typctxtwo} = \sizetyp{\mtypetwo}$. Then $\tderiv \tderiveq \tderivtwo$ and 
$\sizem{\tderivtwo} = 0 = \sizectx{\typctxtwo} - \sizetyp{\mtypetwo}$.
		

		%%%%%%%%%%%%%%%%%
		\item \emph{Inert application}, \ie $\tm = \sitm \sfire$. Then $\tderiv$ ends with rule $\ruleAp$. Let 
$\tderiv_{\sitm}$ and $\tderiv_{\sfire}$ be its two premises. 		
		By \ih, there is a derivation $\concl{\tderivtwo_{\sfire}}{\typctxtwo_{\sfire}}{\sfire}{\mtypethree}$ such that 
$\tderivtwo_{\sfire} \tderiveq \tderiv_{\sfire}$ and $\sizem{\tderiv_{\sfire}} =  
\sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypethree}$.
		Let $\mtypetwo$ be a multi type such that $\card\mtypetwo = \card\mtype$. Note that rule $\ruleAp$ forces the multi 
type assigned by $\tderiv_{\sitm}$ to $\sitm$ to be a singleton. By \ih, there is a derivation 
$\concl{\tderivtwo_{\sitm}}{\typctxtwo_{\sitm}}{\sitm}{\mset{\larrow{\mtypethree}{\mtypetwo}}}$ such that 
$\tderivtwo_{\sitm} \tderiveq \tderiv_{\sitm}$ and $ 
\sizem{\tderiv_{\sitm}} = \sizectx{\typctxtwo_{\sitm}} - \sizetyp{\mset{\larrow{\mtypethree}{\mtypetwo}}} = 
\sizectx{\typctxtwo_{\sitm}} - 
\sizetyp{\mtypethree} - \sizetyp{\mtypetwo} - 1$.
		We have the following derivation $\tderivtwo$:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctxtwo_{\sitm} \vdash \sitm \hastype \mset{\larrow{\mtypethree}{\mtypetwo}}}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sfire}$}{\typctxtwo_{\sfire} \vdash \sfire \hastype \mtypethree}
		\infer2[\footnotesize$\ruleAp$]{\typctxtwo_{\sitm}\mplus\typctxtwo_{\sfire} \vdash \sitm\sfire \hastype \mtypetwo}
		\end{prooftree}
		\end{equation*}
		Clearly, $\tderiv \tderiveq \tderivtwo$. Let  $\typctxtwo \defeq \typctxtwo_{\sitm}\mplus\typctxtwo_{\sfire}$. Then 
		\[\small\begin{array}{rcl}
			\sizem\tderiv &= &\sizem{\tderiv_{\sitm}}+ \sizem{\tderiv_{\sfire}} 
+ 1 
			\\
			& =_{\ih} & \sizem{\tderiv_{\sitm}} + \sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypethree} +1
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sitm}} - 
\sizetyp{\mtypethree} - \sizetyp{\mtypetwo} - 1 + \sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypethree} +1
			\\
			& = & \sizectx{\typctxtwo_{\sitm}} + \sizectx{\typctxtwo_{\sfire}} - \sizetyp{\mtypetwo}
			\\
			& = &
			\sizectx\typctxtwo - \sizetyp{\mtypetwo}
		\end{array}\]
		
		For point 2, we use point 1 with $\mtypetwo \defeq \mset{\ground_1, \ldots, \ground_{\card\mtype}}$, for which 
$\sizetyp{\mtypetwo} = 0$, so that equation $\sizem{\tderiv} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo}$ also 
holds true. 
				
		%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on inert}, \ie $\tm = \sitm \esub{\var}{\sitmtwo}$.
		Then $\tderiv$ ends with rule $\ruleES$. Let $\tderiv_{\sitm}$ and $\tderiv_{\sitmtwo}$ be its two premises and Let 
$\mtypetwo$ be a multi type such that $\card\mtypetwo = \card\mtype$.
		By \ih, there is a derivation $\concl{\tderivtwo_{\sitm}}{\typctxtwo_{\sitm}, 
\var\hastype\mtypethree}{\sitm}{\mtypetwo}$ such that $\tderivtwo_{\sitm} \tderiveq \tderiv_{\sitm}$ and 
$\sizem{\tderiv_{\sitm}} = \sizectx{\typctxtwo_{\sitm}, \var\hastype\mtypethree } - \sizetyp{\mtypetwo} = 
\sizectx{\typctxtwo_{\sitm}} + \sizetyp{\mtypethree} - \sizetyp{\mtypetwo}$. By 
\reflemma{skel-equiv-properties}, $\mtypethree$ has the same cardinality of the type $\mtypethree'$ given by 
$\tderiv_{\sitm}$ to $\var$, which is also the same type given by $\tderiv_{\sitmtwo}$ to $\sitmtwo$. We can then apply 
the \ih and obtain a derivation $\concl{\tderivtwo_{\sitmtwo}}{\typctxtwo_{\sitmtwo}}{\sitmtwo}{\mtypethree}$ such that 
$\tderivtwo_{\sitmtwo} \tderiveq \tderiv_{\sitmtwo}$ and $\sizem{\tderiv_{\sitmtwo}} = 
\sizectx{\typctxtwo_{\sitmtwo}} - \sizetyp{\mtypethree}$.
		We have the following derivation $\tderivtwo$:
				\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctxtwo_{\sitm}, \var\hastype\mtypethree \vdash \sitm \hastype \mtypetwo}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitmtwo}$}{\typctxtwo_{\sitmtwo} \vdash \sitmtwo \hastype \mtypethree}
		\infer2[\footnotesize$\ruleES$]{\typctxtwo_{\sitm} \mplus \typctxtwo_{\sitmtwo} \vdash \sitm \esub{\var}{\sitmtwo} 
\hastype \mtypetwo}
		\end{prooftree}
		\end{equation*}
Clearly, $\tderiv \tderiveq \tderivtwo$. Let  $\typctxtwo \defeq \typctxtwo_{\sitmtwo}\mplus\typctxtwo_{\sitm}$. Then 
		\[\small\begin{array}{rcl}
			\sizem\tderiv &=&\sizem{\tderiv_{\sitm}}+ \sizem{\tderiv_{\sitmtwo}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sitm}} + \sizetyp{\mtypethree} - \sizetyp{\mtypetwo} + 
\sizem{\tderiv_{\sitmtwo}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sitm}} + \sizetyp{\mtypethree} - \sizetyp{\mtypetwo} + 
\sizectx{\typctxtwo_{\sitmtwo}} - \sizetyp{\mtypethree} 
			\\
			& = & \sizectx{\typctxtwo_{\sitmtwo}} + \sizectx{\typctxtwo_{\sitm}} - \sizetyp{\mtypetwo}
			\\
			& = &
			\sizectx\typctxtwo - \sizetyp{\mtypetwo}
		\end{array}\]		
				For point 2, we use point 1 with $\mtypetwo \defeq \mset{\ground_1, \ldots, \ground_{\card\mtype}}$, for which 
$\sizetyp{\mtypetwo} = 0$, so that equation $\sizem{\tderiv} = \sizectx{\typctxtwo} + \sizetyp{\mtypetwo}$ also 
holds true. 


		%%%%%%%%%%%%%%%%%		
		\item \emph{Abstraction}, \ie $\sfire = \la{\var}{\sfiretwo}$. 
		Then $\tderiv$ ends with a rule $\ruleManyVal$ with $n$ premises, each one ending with a $\ruleFun$ rule. Let 
$\tderiv^i$ be the premise of the $\ruleFun$ rule of the $i$-th derivation above the $\ruleManyVal$ rule, for 
$i\in\set{1,\ldots,n} \eqdef I$.
		By \ih, there exists a derivation $\concl{\tderivtwo^i}{\typctxtwo_i, \var \hastype 
\mtypethree_i'}{\sfiretwo}{\mtypethree_i}$ such that $\tderivtwo^i \tderiveq \tderiv^i$ and $\sizem{\tderiv^i} = 
\sizectx{\typctxtwo_i} + \sizetyp{\mtypethree_i} + \sizetyp{\mtypethree_i'}$.
		We have the following derivation:
		\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo^i$}{\typctxtwo_i, \var \hastype \mtypethree_i' \vdash \sfiretwo \hastype \mtypethree_i}
		
		\infer1[\footnotesize$\lambda$]{\typctxtwo_i \vdash \la{\var}\sfiretwo \hastype 
\larrow{\mtypethree'_i}{\mtypethree_i}}
		\delims{\left[}{\right]_{\iI}}
		\infer1[\footnotesize$\ruleManyVal$]{\uplus_{\iI}\typctxtwo_i \vdash \la{\var}\sfiretwo \hastype 
\mset{\larrow{\mtypethree'_i}{\mtypethree_i}}_{\iI}}		\end{prooftree}
		\end{equation*}
		Clearly, $\tderiv \tderiveq \tderivtwo$. Let $\typctxtwo \defeq \uplus_{\iI}\typctxtwo_i$ and $ \mtypetwo \defeq 
\mset{\larrow{\mtypethree'_i}{\mtypethree_i}}_{\iI}$. We have:
		\[\small\begin{array}{rcl}
			\sizem\tderiv &= &n+\sum_{\iI} \sizem{\tderiv^i}
			\\
			& =_{\ih} & n+\sum_{\iI}(\sizectx{\typctxtwo_i} + \sizetyp{\mtypethree_i} + \sizetyp{\mtypethree_i'}) 
			\\
			& = & \sum_{\iI}\sizectx{\typctxtwo_i} + (n+\sum_{\iI}(\sizetyp{\mtypethree_i} + \sizetyp{\mtypethree_i'}))
			\\
			& = & \sizectx\typctxtwo + \sizetyp{\mset{\larrow{\mtypethree'_i}{\mtypethree_i}}_{\iI}}
			\\
			& = & \sizectx\typctxtwo + \sizetyp\mtypetwo
		\end{array}\]
				
		
		%%%%%%%%%%%%%%%%%%%%%%%
		\item \emph{Explicit substitution on fireball}, \ie $\tm = \sfire \esub{\var}{\sitm}$.
		Then $\tderiv$ ends with rule $\ruleES$. Let $\tderiv_{\sfire}$ and $\tderiv_{\sitm}$ be its two premises. 
		By \ih, there is a derivation $\concl{\tderivtwo_{\sfire}}{\typctxtwo_{\sfire}, 
\var\hastype\mtypethree}{\sfire}{\mtypetwo}$ such that $\tderivtwo_{\sfire} \tderiveq \tderiv_{\sfire}$ and 
$\sizem{\tderiv_{\sfire}} = \sizectx{\typctxtwo_{\sfire}} + \size{\mtypethree} + \sizetyp{\mtypetwo}$. By 
\reflemma{skel-equiv-properties}, $\mtypethree$ has the same cardinality of the type $\mtypethree'$ given by 
$\tderiv_{\sfire}$ to $\var$, which is also the same type given by $\tderiv_{\sitm}$ to $\sitm$.
		By \ih, there is a derivation $\concl{\tderivtwo_{\sitm}}{\typctxtwo_{\sitm}}{\sitm}{\mtypethree}$ such that 
$\tderivtwo_{\sitm} \tderiveq \tderiv_{\sitm}$ and $\sizem{\tderiv_{\sitm}} = 
\sizectx{\typctxtwo_{\sitm}} - \sizetyp{\mtypethree}$.
		We have the following derivation $\tderivtwo$:
				\begin{equation*}
		\tderivtwo \defeq 
		\begin{prooftree}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sfire}$}{\typctxtwo_{\sfire}, \var\hastype\mtypethree \vdash \sfire \hastype \mtypetwo}
		\hypo{}
		\ellipsis{$\tderivtwo_{\sitm}$}{\typctxtwo_{\sitm} \vdash \sitm \hastype \mtypethree}
		\infer2[\footnotesize$\ruleES$]{\typctxtwo_{\sfire} \mplus \typctxtwo_{\sitm} \vdash \sfire \esub{\var}{\sitm} 
\hastype \mtypetwo}
		\end{prooftree}
		\end{equation*}
	Clearly, $\tderiv \tderiveq \tderivtwo$. Let  $\typctxtwo \defeq \typctxtwo_{\sitm}\mplus\typctxtwo_{\sfire}$. Then 
		\[\begin{array}{rcl}
			\sizem\tderiv &= & \sizem{\tderiv_{\sfire}}+ \sizem{\tderiv_{\sitm}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sfire}} + \size{\mtypethree} + \sizetyp{\mtypetwo} + \sizem{\tderiv_{\sitm}} 
			\\
			& =_{\ih} & \sizectx{\typctxtwo_{\sfire}} + \size{\mtypethree} + \sizetyp{\mtypetwo} + 
\sizectx{\typctxtwo_{\sitm}} 
-\sizetyp{\mtypethree}  
			\\
			& = & \sizectx{\typctxtwo_{\sitm}} + \sizectx{\typctxtwo_{\sfire}} + \sizetyp{\mtypetwo}
			\\
			& = &
			\sizectx\typctxtwo + \sizetyp{\mtypetwo}
		\end{array}\]
\qedhere
	\end{itemize}	
\end{proof}


==> proofs/weak_composable_bounds.tex <==
% !TEX root = ../main.tex
\begin{proof}
	By shrinking completeness (\refthm{shrinking-characterization}), there is a derivation $\derive{\tderiv}{\nf\nftwo}$ with $2\size{\deriv} + \sksize{\nfthree} = \insize{\tderiv}$. 
	The last rule of $\tderiv$ is an $\ruleAp$ rule between two derivations 
	$\tderiv_\nf$ and $\tderiv_{\nftwo}$. Note that $\insize{\tderiv} = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1$. 
		By dry representation (\refthmp{dry_representation}{core}), there are dry derivations $\concl{\tderiv_\nf'}{\,}{\nf}{\ltype}$ and $\concl{\tderiv_{\nftwo}'}{\,}{\nftwo}{\mtype}$ such that $\tderiv_\nf \tderiveq \tderiv_\nf'$ and $\tderiv_{\nftwo} \tderiveq \tderiv_{\nftwo}'$. By the properties of skeletal invariants (\reflemma{skel-equiv-properties}), $\insize{\tderiv_\nf} = \insize{\tderiv_\nf'}$ and $\insize{\tderiv_{\nftwo}} = \insize{\tderiv_{\nftwo}'}$. By the fact that dry derivations have minimal types (\refprop{dry_is_minimal}), $\insize{\tderiv_\nf'}= \size\ltype$ and $\insize{\tderiv_{\nftwo}'}= \size\mtype$. Putting it all together, we obtain $2\size{\deriv} + \sksize{\nfthree} = \insize{\tderiv_\nf} + \insize{\tderiv_{\nftwo}} + 1 = \size\ltype+\size\mtype+1$ with $\ltype\in \sem\nf$ and $\mtype\in\sem\nftwo$.	
\end{proof}
